Cross-View Tracking for Multi-Human 3D Pose Estimation at over 100 FPS

Estimating 3D poses of multiple humans in real-time is a classic but still challenging task in computer vision. Its major difficulty lies in the ambiguity in cross-view association of 2D poses and the huge state space when there are multiple people in multiple views. In this paper, we present a novel solution for multi-human 3D pose estimation from multiple calibrated camera views. It takes 2D poses in different camera coordinates as inputs and aims for the accurate 3D poses in the global coordinate. Unlike previous methods that associate 2D poses among all pairs of views from scratch at every frame, we exploit the temporal consistency in videos to match the 2D inputs with 3D poses directly in 3-space. More specifically, we propose to retain the 3D pose for each person and update them iteratively via the cross-view multi-human tracking. This novel formulation improves both accuracy and efficiency, as we demonstrated on widely-used public datasets. To further verify the scalability of our method, we propose a new large-scale multi-human dataset with 12 to 28 camera views. Without bells and whistles, our solution achieves 154 FPS on 12 cameras and 34 FPS on 28 cameras, indicating its ability to handle large-scale real-world applications. The proposed dataset is released at https://github.com/longcw/crossview_3d_pose_tracking.

==> draft.tex <==


There are at least two advantages from our modification:
1) the strict synchronization between cameras 
is no longer required;
and 2) the overall computational cost increases
linearly as the number of cameras increases,
which makes our framework has the potential
to be applied for large-scale camera network.



The iterative processing 
enables the potential of 
deployment of our framework in a large-scale camera network.






There are at least two advantages from the iterative processing:
1) the strict synchronization between cameras 
is no longer required;
2) the overall computational cost only increases
linearly as the number of cameras increases.



Such a modification is not trivial,

Taking inputs iteratively for multi-human 3D pose estimation
is nontrivial and 

challenges

Treating the inputs in this way,
% only one camera view is processed at one time,
inputs from multiple cameras are processed iteratively,
making the computational complexity
of the overall system increases linearly
as the number of cameras increases.

The framework is composed of 

The task of the cross-view tracker is to


along with the detected 2D joints and the metadata
such as timestamp and camera index.

% Such a modification brings two advantages:
% 1) the strict synchronization between cameras 
% is no longer required;
% and 2) the overall computational cost increases
% linearly as the number of cameras increases,
% which makes our framework has the potential
% to be applied for large-scale camera network.
% 
